Occlusion resistant learning of intuitive physics from videos

To reach human performance on complex tasks, a key ability for artificial systems is to understand physical interactions between objects, and predict future outcomes of a situation. This ability, often referred to as intuitive physics, has recently received attention and several methods were proposed to learn these physical rules from video sequences. Yet, most of these methods are restricted to the case where no, or only limited, occlusions occur. In this work we propose a probabilistic formulation of learning intuitive physics in 3D scenes with significant inter-object occlusions. In our formulation, object positions are modeled as latent variables enabling the reconstruction of the scene. We then propose a series of approximations that make this problem tractable. Object proposals are linked across frames using a combination of a recurrent interaction network, modeling the physics in object space, and a compositional renderer, modeling the way in which objects project onto pixel space. We demonstrate significant improvements over state-of-the-art in the intuitive physics benchmark of IntPhys. We apply our method to a second dataset with increasing levels of occlusions, showing it realistically predicts segmentation masks up to 30 frames in the future. Finally, we also show results on predicting motion of objects in real videos.

==> ICML2020- Towards Occlusion resistant learning of intuitive physics from videos (Ronan et al)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> ICML2020- Towards Occlusion resistant learning of intuitive physics from videos (Ronan et al)/suppmat.tex <==
\title{Supplementary material}

\author{}
\date{}

\maketitle

This supplementary material: (i) describes the provided supplementary videos (section~\ref{sec:videos}), (ii) provides additional training details (section~\ref{sec:training}), (iii) explains in more depth the \textit{event decoding} procedure defined in section 3.4 in the main paper (section~\ref{sec:decoding}) (iv) gives details of the datasets used in the subsection 4.2 (section~\ref{sec:datasets}), (v) provides additional ablation studies and comparisons with baselines (sections~\ref{ablation},~\ref{sec:rollout},~\ref{sec:real},~\ref{sec:pixelerror}). 

\section{ Description of supplementary videos}
\label{sec:videos}

In this section we present qualitative results of our method on different datasets. We first show videos from IntPhys benchmark, where inferred object states are depicted onto observed frames. Then we show differents outputs on the pybullet datasets, for different levels of occlusions. Finally we present examples of predictions from our Recurrent Interaction Network on real scenes.

The videos are in the google drive: \url{https://drive.google.com/open?id=1Qc8flIAxUGzfRfeFyyUEGXe6J5AUGUjE} in the \texttt{videos/} subdirectory. Please see also the \texttt{README} slideshow in the same directory.

\subsection{IntPhys benchmark}

The Intphys Benchmark consists in a set of video clips in a virtual environment. Half of the videos are possible event and half are impossible, the goal being to discriminate the two.

In the following we show impossible events, along with outputs of our event decoding method. Our dynamics and rendering models predict future frames (masks) in the videos, which are compared with the observed masks (pre-trained detector). This allows us to derive a plausibility loss used to discriminate possible and impossible events (see section 4.1).

\begin{itemize}
 \item \textbf{occluded\_impossible\_*.mp4} show examples of impossible videos from the IntPhys benchmark, along with visualization of our method. Each video contains four splits; on \underline{top/left} is shown the raw input frame; on \underline{bottom/left} is the mask obtained from the raw frame with the pre-trained mask detector (which we call \textit{observed mask}); on \underline{top/right} is the raw frame with superimposed output physical states predicted by our method; on \underline{bottom/right} is the reconstructed mask obtained with the Compositional Renderer (which we call \textit{predicted mask}). Throughout the sequence, our method predicts the full trajectory of objects. When an object should be visible (i.e. not behind an occluder), the renderer predicts correctly its mask. If at the same time the object has disappeared from the observed mask, or changed too much in position or shape, it causes a mismatch between the predicted and the observed masks, hence a higher plausibility loss. This plausibility loss is use for the classification task of IntPhys benchmark (see quantitative results in main paper, section 4.1).
 \item \textbf{visible\_impossible\_*.mp4} show similar videos but with impossible events occurring in the "visible" (easier) task of the IntPhys benchmark. 
 \item \textbf{intphys\_*.mp4} show object following in the IntPhys training set.
 \end{itemize}
 
\subsection{Pybullet experiments}
 
 We present qualitative results on our Pybullet dataset. We construct videos including a various number of objects with different points of view and increasing levels of camera tilts introducing inter-object occlusions. First, we show predicted physical states drawn on object states, to demonstrate the ability of the method to track objects under occlusions. Then we show videos of long rollouts where, from one pair of input frames, we predict a full trajectory and render masks with the Compositional Neural Renderer.
 
 
 \begin{itemize}
 \item \textbf{scene\_overview.mp4} shows raw videos of the entire environment.
 \item \textbf{tracking\_occlusions\_*.mp4} show examples of position prediction through complete occlusions, using our event decoding procedure. This shows that our model can keep track of the object identity through complete occlusions, mimicking ``object permanence".
 \item \textbf{one\_class*.mp4} show different examples of our model following motion of multiple objects in the scene. All balls have the same color which makes them difficult to follow in case of mutual interactions. Videos come from tilted \ang{25} experiments, which are the most challenging because they include inter-object occlusions. Dots represent the predicted position of each object, the color being its identity. Our model shows very good predictions with small colored markers (dots) well centered in the middle of each object, with marker color remaining constant for each object preserving the object identity during occlusions and collisions. \textbf{one\_class\_raw*.mp4} show rendered original views of the same dynamic scenes but imaged from a different viewpoint for better understanding.
 \item \textbf{rollout\_0.mp4}, \textbf{rollout\_1.mp4} show three different prediction roll-outs of the Recurrent Interaction Network (without event decoding procedure). From left to right: ground truth trajectories, our model trained of state, our model trained on masks, our model trained on masks with occlusions during training. Rollout length is 20 frames.
 \item \textbf{rollout\_tilt*\_model.mp4} and \textbf{rollout\_tilt*\_groundtruth.mp4} show the same dynamic scene but observed with various camera tilts (e.g. \textbf{tilt45\_model.mp4} show a video for a camera tilt of 45 degrees). \textbf{*\_model.mp4} are predicted roll-outs of our Recurrent Interaction Network ($RecIntNet$), without event decoding. \textbf{*\_groundtruth.mp4} are the corresponding ground-truth trajectories, rendered with the \textit{Compositional Rendering Network}.
 \item \textbf{rollout\_pybullet\_*.mp4} show free roll-outs (no event decoding) on synthetic dataset.
 \end{itemize}
 
 \subsection{Real videos}
 
 \begin{itemize}
 \item \textbf{rollout\_real\_*.mp4} show generalization to real scenes.
\end{itemize}

\section{ Training details}
\label{sec:training}

This section gives details of the offline pre-training of the Compositional Rendering Network and detailed outline of the algorithm for training the Recurrent Interaction Network.

\paragraph{Pre-Training the Compositional Rendering Network.} We train the neural renderer to predict mask and depth $\hat{M}_t,\hat{D}_t$ from a list of objects $[p_x,p_y,d,\bm{c}]$ where
$p_x,p_y$ are x-y coordinates of the object in the frame, $d$ is the distance between the object and the camera and $\bm{c}$ is a vector for intrinsic object properties containing the size of the object, its class (in our experiments a binary variable for whether the object is a ball, a square or an occluder) and its color as vector in $[0,1]^3$. In IntPhys benchmark, occluders are not modeled with a single point $[p_x,p_y,d,\bm{c}]$ but with four points $[p_x^k,p_y^k,d^k],k=1..4$ corresponding to the four corners of the quadrilateral. These four corners are computed from the occluder instance mask, after detecting contours and applying Ramer–Douglas–Peucker algorithm to approximate the shape with a quadrilateral.

The target mask is a $128\times128$ image where each pixel value indicates the index of the corresponding object mask (0 for the background, $i\in{1..N}$ for objects). The loss on the mask is negative log-likelihood, which corresponds to the average classification loss on each pixel
\begin{align}
\small
 L_{\text{mask}}(\hat{M}, M) = \sum_{i \leq h, j \leq w} \sum_{n \leq N} \bm{1}(M_{i,j}=n)log(\hat{M}_{i,j,n}),
 \label{eq:lossmask}
\end{align}
where the first sum is over individual pixels indexed by $i$ and $j$, the second sum is over the individual objects indexed by $n$, $\forall \hat{M} \in [0,1]^{h\times w\times N}$ are the predicted (soft-) object masks, and $\forall M \in [\![1,N[\!]^{h \times w}$ is the scene ground truth mask containing all objects. 

The target depth map is a $128\times128$ image with values being normalized to the [-1,1] interval during training. The loss on the depth map prediction is the mean squared error
\begin{align}
 L_{\text{depth}}(\hat{D}, D) = \sum_{i \leq h, j \leq w} (\hat{D}_{i,j} - D_{i,j})^2, 
 \label{eq:lossdepth}
\end{align}
where $\forall \hat{D}$ and $D \in \mathbb{R}^{h\times w}$ are the predicted and ground truth depth maps, respectively. 
The final loss used to train the renderer is the weighted sum of losses on masks and depth maps, $L = 0.7 * L_{mask} + 0.3 * L_{depth}$. We use the \texttt{Adam} optimizer with default parameters, and reduce learning rate by a factor $10$ each time the loss on the validation set does not decrease during $10$ epochs. We pre-train the network on a separate set of 15000 images generated with \texttt{pybullet} and containing similar objects as in our videos.

\paragraph{Training details of the Recurrent Interaction Network.}

From a sequence of L frames with their instance masks we compute objects position, size and shape (see section 3.2 in the main body). Initial velocities of objects are estimated as the position deltas between the first two positions. This initial state (position, velocity, size and shape of all objects) is given as input of the Recurrent Interaction Network to predict the next L-2 states. The predicted L-2 positions are compared with observed object positions. The sum of prediction errors (section 3.3 in core paper) is used as loss to train parameters of the Recurrent Interaction Network. Optimization is done via gradient descent, using Adam with learning rate $1e-3$, reducing learning by a factor of 10 each time loss on validation plateaus during 10 epochs. We tried several sequence lengths ($4$, $6$, $10$), $10$ giving the most stable results. During such sequence, when an object was occluded (thus position not being observed), we set its loss to zero. 

\section{Event Decoding}
\label{sec:decoding}

The detailed outline of the event decoding procedure described in section \ref{sec:decoding} of the main paper is given in Algorithm~\ref{alg:procedure}.  Two example figures (Figure \ref{fig:decoding_1} \& \ref{fig:decoding_2}) gives an intuition behind the \textit{render} and \textit{physics} losses.

\begin{figure*}[h!]
\begin{center}
\includegraphics[width=1\linewidth]{example_1.pdf}
\caption{{\bf Video example from the IntPhys benchmark.} Four frames from a video in block \texttt{O1}, with superimposed heatmaps. Heatmaps (colored blobs) correspond to the difference, per pixel, between the predicted and the observed object mask. In these video, a cube moves from left to right  but disappears behind the occluder. The Recurrent Interaction Network predicts correctly its motion behind the occluder and the Compositional Renderer reconstructs its mask. The fact that the object is absent in the observed mask leads to a large \textit{render} loss, illustrated by the high heatmap values (violet) at the position where the ball is expected to be. }
\label{fig:decoding_1}
\end{center}
\end{figure*}

\begin{figure*}[h!]
\begin{center}
\includegraphics[width=0.75\linewidth]{example_2.pdf}
\caption{{\bf Video example from the IntPhys benchmark.} Three frames from a video in block \texttt{O2}, where an object "jumps" from one place to another. The graph proposal phase returns the right trajectory of the object but the Recurrent Interaction Network returns a high \textit{physics} loss at the moment of the jump, because the observed position is far from the predicted one.}
\label{fig:decoding_2}
\end{center}
\end{figure*}

\begin{algorithm}[tbp]
\small
\SetAlgoLined
\KwData{\\
\Indp $T$: length of the video\;\\
$f_t,m_t~t=1..T$: videos frames, segmentation masks\;\\
\texttt{Detection($m_t$)}: returns centroid and size of instance masks\;\\
\texttt{RecIntNet}: Pre-trained Recurrent Interaction Network\;\\
\texttt{Rend}: Pre-trained Neural Renderer\;\\
\texttt{ClosestMatch(a,b)}: for a, b two lists of objects, computes the optimal ordering of elements in b to match those in a \;\\
$0 < \lambda < 1$: weighting physical and visual losses\;\\
}
\KwResult{\\
\Indp Estimated states $s_{1...T}$\;\\
Plausibility loss for the video\;\\
}
\vspace{0.7cm}
\textbf{Initialization}:\\
 $d_{t=1..T} = \text{Detection}(f_t)$\;
 $n_t \leftarrow (\#\{d_t\}, \text{mean}_t\textit{size}(d_t)$) \;\\
 $t^* \leftarrow \argmax_{t}({n_t + n_{t+1}})$\;\\
 \CommentSty{//$(t^*,t^*+1)$ is the pair of frames containing the maximum number of objects (with the max number of visible pixels in case of equality).}\\
 ($p_{t^*},p_{t^*+1}) \leftarrow (d_{t^*}, \text{ClosestMatch}(d_{t^*}, d_{t^*+1}))$\;\\
 \CommentSty{//Rearange $d_{t^*+1}$ to have same object ordering as in $d_{t^*}$}.\\

\textbf{Graph Proposal}:\\
\CommentSty{//$t^*$ is a good starting point for parsing the scene (because we observe most of the objects during two consecutive frames). We use RecIntNet to predict the next position of each object, which we link to an object detection. Repeating this step until the end of the video returns object trajectory candidates.}\\
$v_{t^*+1} \leftarrow p_{t^*+1} - p_{t^*}$\;\\
$s_{t^*+1} \leftarrow [p_{t^*+1},v_{t^*+1}]$\;\\
\For{$t \in \{t^*+1,..,T\}$}{ 
 $\hat{s}_{t+1} \leftarrow \text{RecIntNet}(s_t)$\;\\
 $s_{t+1} \leftarrow \text{ClosestMatch}(\hat{s}_{t+1}, d_{t+1})$\;\\
}
\CommentSty{//Backward: do the same from $t^*$ to 1.}
\\
\textbf{Differentiable optimization}:\\
 \CommentSty{//$\hat{s}_{t=1..T}$ is a sequence of physical states. At every time step $t$ it contains the position, velocity, size and shape of all objects, in the same order. Due to occlusions and detection errors, it is sub-optimal and can be refined to minimize equation 3 in the main paper.}\\
$\text{Loss}_\text{physics}(s) \leftarrow \sum_{t=1}^T \|\hat{s}_{t+1} - s_{t+1}\|^2$\;\\
$\text{Loss}_\text{visual}(s) \leftarrow \sum_{t=1}^T \texttt{NLL}(\texttt{Rend}(s_t), m_t)$\;\\
$\text{Loss}_\text{plausibility}(s) \leftarrow \lambda\text{Loss}_\text{physics}(s) + (1-\lambda)\text{Loss}_\text{visual}(s)$\;
 $(\text{Estimated states}, \text{plausibility loss}) \leftarrow \texttt{SGD}_s(\text{Loss}_\text{plausibility}(s))$\;
 \\\CommentSty{//with $lr=1e-3$ and $n_\text{steps}=1000$}\;

\caption{{\bf Event decoding procedure}}
\label{alg:procedure}
\end{algorithm}


\section{ Datasets}
\label{sec:datasets}

\begin{figure*}[h!]
\begin{center}
\includegraphics[width=1\linewidth]{picture.pdf}
\end{center}
\caption{ Sample video frames (instance mask + depth field) from our datasets (top) together with predictions obtained by our model (bottom). Taken from the top-view, occluded and tilted experiments. {\bf Please see additional video results in the google drive \url{https://drive.google.com/open?id=1Qc8flIAxUGzfRfeFyyUEGXe6J5AUGUjE}.}}
\end{figure*}

To validate our model, we use pybullet\footnote{\url{https://pypi.org/project/pybullet}} physics simulator to generate videos of variable number of balls of different colors and sizes bouncing in a 3D scene (a large box with solid walls) containing a variable number of smaller static 3D boxes. We generate five dataset versions, where we vary the camera tilt and the presence of occluders. All experiments are made with datasets of 12,000 videos of 30 frames (with a frame rate of 20 frames per second). For each dataset, we keep 2,000 videos separate to pre-train the renderer, $9,000$ videos to train the physics predictor and $1,000$ videos for evaluation. Our scene contains a variable number of balls (up to 6) with random initial positions and velocities, bouncing against each other and the walls. Initial positions are sampled from a uniform distribution in the box $[1,200]^2$, all balls lying on the ground. Initial velocities along $x$ and $y$ axes are sampled in $\textit{Unif}([-25,25])$ units per frame, initial velocity along $z$-axis is set to $0$. The radius of each ball is sampled uniformly in $[10,40]$. Scenes also contain a variable number of boxes (up to 2) fixed to the floor, against which balls can collide. Contrary to \cite{battaglia_interaction_2016} where authors set a frame rate of 1000 frames per second, we sample 30 frames per second, which is more reasonable when working with masks (because of the computation cost of mask prediction).

\paragraph{Top-view.}
In the first dataset we record videos with a top camera view, where the borders of the frame coincide with the walls of the box. Here, initial motion is orthogonal to the camera, which makes this dataset very similar to the 2D bouncing balls datasets presented in \cite{battaglia_interaction_2016} and \cite{watters_visual_2017}. However, our dataset is 3D and because of collisions and the fact that the balls have different sizes, balls can jump on top of each other, making occlusions possible, even if not frequent. 

\paragraph{Top-view with Occlusions.}
To test the ability of our method to learn object dynamics in environments where occlusions occur frequently, we record the second dataset including frequent occlusions. We add an occluder to the scene, which is an object of irregular shape (an airplane), occluding $25\%$ of the frame and moving in 3D between the balls and the camera. This occluder has a rectilinear motion and goes from the bottom to the top of the frame during the whole video sequence. Sample frames and rendered predictions can be found in the supplementary material.

\paragraph{Tilted-views.}
In three additional datasets we keep the same objects and motions but tilt the camera with angles of \ang{45}, \ang{65} and \ang{75} degrees. Increasing the tilt of the camera results in more severe inter-object occlusions (both partial and complete) where the balls pass in front of each other, and in front and behind the static boxes, at different distances to the camera. In addition, the ball trajectories are becoming more complex due to increasing perspective effects.
In contrary to the top-view experiment, the motion is not orthogonal to the camera plane anymore, and depth becomes crucial to predict the future motion.

\section{Ablation studies}
\label{ablation}

For the purpose of comparison, we also evaluate three models trained using ground truth object states. Results are shown in table \label{ref:gtposerror}. Our Recurrent Interaction Network trained on ground truth object states gives similar results to the model of~\cite{battaglia_interaction_2016}. As expected, training on ground truth states (effectively ignoring occlusions and other effects) performs better than training from object masks and depth.
\begin{table}[h]
\footnotesize
\begin{center}
\begin{tabular}{lrrrr}
\hline
     & Top view & \ang{45} tilt & \ang{25} tilt & \ang{15} tilt \\   
%     & & occlusion & & & \\
     \hline
\multicolumn{5}{c}{}\\
\scriptsize{NoProba-RIN}      & 4.76 / 9.72 & 6.21 / 10.0 & 5.2 / 12.2 & 7.3 / 13.8 \\
RIN     & 4.5 / 9.0 & 6.0 / 9.6 & 5.2 / 12.2 & 7.3 / 13.2 \\
\citeyear{battaglia_interaction_2016}** & 3.6 / 10.1 & 4.5 / 9.9 & 4.5 / 11.0 & 5.3 / 12.3\\
\hline
\end{tabular}
\end{center}
\caption{Average Euclidean (L2) distance (in an untilted 200x200x200 reference Cartesian coordinate system) between predicted and ground truth positions, for a prediction horizon of 5 frames / 10 frames, trained on ground truth positions. **\cite{battaglia_interaction_2016} is trained with more supervision, since target values include ground truth velocities, not available to other methods.
}
\label{tab:gtposerror}
\end{table}

\section{Roll-out results}
\label{sec:rollout}

We evaluate our model on \textit{object following}, applying an online variant of the scene decoding procedure detailed in \ref{sec:decoding}. This online variant consists in applying the state optimization sequentially (as new frames arrive), instead of on the full sequence. For each new frame, the state prediction $\hat{s}_{t+1}$ given by $RecIntNet$ is used to predict a resulting mask. This mask is compared to the observation, and we apply directly the final step in Algorithm \ref{alg:procedure} (Differentiable optimization). It consists in minimizing  $\lambda\text{Loss}_\text{physics}(s) + (1-\lambda)\text{Loss}_\text{visual}(s)$ via gradient descent over the state $s$. During full occlusion, the position is solely determined by $RecIntNet$, since $\text{Loss}_\text{render}$ has a zero gradient. When the object is completely or partially visible, the $\text{Loss}_\text{render}$ in the minimization make the predicted state closer to its observed value. To test object following, we measure the accuracy of the position estimates across long sequences (up to 30 frames) containing occlusions. 
Table \ref{tab:tracking} shows the percentage of object predictions that diverge by more than an object diameter (20 pixels) using this method. The performance is very good, even for tilted views. In Figure \ref{fig:tracking}, we report the proportion of correctly followed objects for different rollout lengths (5, 10 and 30 frames) as a function of the distance error (pixels). Note that the size of the smallest object is around 20 pixels.

\begin{table}[h]
\begin{center}
\begin{tabular}{lccccc}
\hline
Synthetic videos & 5 fr. & 10 fr. & 30 fr. \\
\hline
 Ours, top view & 100 & 100 & 100  \\
 Ours, \ang{45} tilt & 99.3 & 96.2 & 96.2  \\
 Ours, \ang{25} tilt & 99.3 & 90.1 & 90.1  \\
 Linear motion baseline & 81.1 & 67.8 & 59.7 \\
\hline
\end{tabular}
\end{center}
\caption{Percentage of predictions within a 20-pixel neighborhood around the target as a function of rollout length measured by the number of frames. 20 pixels corresponds to the size of the smallest objects in the dataset.}
\label{tab:tracking}
\end{table}


\begin{figure}
\centering
\begin{subfigure}{.45\textwidth}
 \centering
 \includegraphics[width=1\linewidth]{one_class_5.pdf}
\end{subfigure}
\begin{subfigure}{.45\textwidth}
 \centering
 \includegraphics[width=1\linewidth]{one_class_10.pdf}
\end{subfigure}
\begin{subfigure}{.45\textwidth}
 \centering
 \includegraphics[width=1\linewidth]{one_class_30.pdf}
\end{subfigure}
\caption{Proportion of correctly followed objects (y-axis) as a function of the distance error in pixels (x-axis) for our approach using online event decoding. The different plots correspond to rollout lengths of 5 (left), 10 (middle) and 30 (right) frames. Different curves correspond to different camera view angles (top-view, tilted 45 degrees and tilted 25 degrees). In this experiment, all objects have the same shape and color making the task of following the same object for a long period of time very challenging. The plots demonstrate the success of our method in this very challenging scenario with object collisions and inter-object occlusions. For example, within a distance threshold of 20 pixels, which corresponds to the size of the smallest objects in the environment, our approach correctly follows more than 90\% of objects during the rollout of 30 frames in all three considered camera viewpoints (top-view, 45 degrees and 25 degrees). {\bf Please see also the supplementary videos ``one\_class*.mp4".}
\label{fig:tracking}
}
\end{figure}


\section{ Experiment with real videos}
\label{sec:real}

We construct a dataset of 22 real videos, containing a variable number of colored balls and blocks in motion. Videos are recorded with a Microsoft Kinect2 device, including RGB and depth frames. The setup is similar to the one generated with Pybullet, recorded with a top camera view and containing 4 balls and a variable number of static blocks (from 0 to 3). Here again, the borders of the frame coincide with the walls of the box.
%
Taking as input object segmentation of the first two frames, we use our model to predict object trajectories through the whole video (see Figure \ref{fig:qualitativeresults}). We use the model trained on top-view synthetic Pybullet videos, without fine-tuning weights. We measure the error between predictions and ground truth positions along the roll-out. Results are shown in Table \ref{tab:realposerror} and clearly demonstrate that out approach outperforms the linear and MLP baselines and makes reasonable predictions on real videos. 


\begin{table}
\small
\begin{center}
\begin{tabular}{lccccc}
\toprule
Model && Linear & MLP & Proba-RecIntNet (ours)\\    
L2 dist. to target && 28/71 & 19/43 & \textbf{12/22} \\
\bottomrule
\end{tabular}
\end{center}
\vspace*{-4mm}
\caption{{\bf Trajectory prediction on real videos.} Average Euclidean (L2) distance (in pixels in a 200 by 200 image) between predicted and ground truth positions, for a prediction horizon of 5 frames / 10 frames.}
\label{tab:realposerror}
\end{table}

\begin{figure*}
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
\includegraphics[width=1\linewidth]{real.png}
\end{center}
\caption{Example of prediction for a real video, with a prediction span of 10 frames. The small colored dots show the predicted positions of objects together with the estimated uncertainty shown by the colored “cloud”. The same colored dot is also shown in the (ground truth) center of each object. The prediction is correct when the two dots coincide. (see \href{https://drive.google.com/open?id=1Qc8flIAxUGzfRfeFyyUEGXe6J5AUGUjE}{additional videos}).}
\label{fig:real}
\end{figure*}

\section{ Future prediction (pixels): Comparison with baselines}
\label{sec:pixelerror}

We evaluate the error of the mask and depth prediction, measured by the training error described in detail in \ref{sec:training}.
Here, we compare our model to a CNN autoencoder~\cite{riochet_intphys:_2018}, which directly predicts future masks from current ones, without explicitly modelling dynamics of the individual objects in the scene. Note this baseline is similar to~\cite{lerer_learning_2016}.
Results are shown in Table S1.
As before, the existence of external occluders or the presence of tilt degrades the performance, but even in this case, our model remains much better than the CNN autoencoder of~\cite{riochet_intphys:_2018}.

\begin{table*}
\small
\begin{center}
\begin{tabular}{lccccc}
\hline
     & Top view & Top view+ & \ang{45} tilt & \ang{25} tilt & \ang{15} tilt \\      
     & & occlusion & & & \\
\hline
CNN autoencoder \cite{riochet_intphys:_2018} & 0.0147 & 0.0451 & 0.0125 & 0.0124 & 0.0121 \\
NoProba-RIN & 0.0101 & 0.0342 & 0.0072 & 0.0070 & 0.0069 \\
Proba-RIN & 0.0100 & 0.0351 & 0.0069 & 0.0071 & 0.0065 \\
\hline
\end{tabular}
\end{center}
\caption*{Aggregate pixel reconstruction error for mask and depth, for a prediction span of two frames. This error is the loss used for training (described in the supplementary material). It is a weighted combination of mask error (per-pixel classification error) and the depth error (mean squared error).}
\label{tab:pixerror}
\end{table*}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

